Can Hallucinations Help? Boosting LLMs for Drug Discovery

Hallucinations in large language models (LLMs), plausible but factually inaccurate text, are often viewed as undesirable. However, recent work suggests that such outputs may hold creative potential. In this paper, we investigate whether hallucinations can improve LLMs on molecule property prediction, a key task in early-stage drug discovery. We prompt LLMs to generate natural language descriptions from molecular SMILES strings and incorporate these often hallucinated descriptions into downstream classification tasks. Evaluating seven instruction-tuned LLMs across five datasets, we find that hallucinations significantly improve predictive accuracy for some models. Notably, Falcon3-Mamba-7B outperforms all baselines when hallucinated text is included, while hallucinations generated by GPT-4o consistently yield the greatest gains between models. We further identify and categorize over 18,000 beneficial hallucinations, with structural misdescriptions emerging as the most impactful type, suggesting that hallucinated statements about molecular structure may increase model confidence. Ablation studies show that larger models benefit more from hallucinations, while temperature has a limited effect. Our findings challenge conventional views of hallucination as purely problematic and suggest new directions for leveraging hallucinations as a useful signal in scientific modeling tasks like drug discovery.

==> table_example_molecule.tex <==
\begin{table*}[ht!]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{@{}p{3cm}p{17cm}@{}}
        \toprule
        \textbf{Name} & \textbf{Description} \\ 
        \midrule
        SMILES & N\#Cc1ccccc1O \\ 
        \midrule
        \addlinespace
        Reference description & The molecule is a nitrile that is hydrogen cyanide in which the hydrogen has been replaced by a hydroxy group. It has a role as an EC 1.2.1.3 [aldehyde dehydrogenase (NAD(+))] inhibitor. It is a nitrile and a member of phenols. It derives from a hydride of a pyridine.\\ 
        \midrule
        \addlinespace
        English & The given molecular formula is N\#Cc1ccccc1O. 

This formula represents a molecule of benzenecarbonitrile, also known as benzonitrile. 

The molecule consists of a benzene ring, which is a planar, ring-shaped structure composed of six carbon atoms, each bonded to a hydrogen atom. 

In this case, one of the carbon atoms in the benzene ring is bonded to a nitrile group (CN), which consists of a carbon atom triple-bonded to a nitrogen atom. 

Additionally, the molecule has an oxygen atom bonded to one of the carbon atoms in the benzene ring, making it a benzonitrile derivative with an alkoxy group (-O-). \\
        \midrule
        \addlinespace
        Chinese & To describe the molecule in Chinese, we first need to identify the chemical structure.

The given chemical formula is N\#Cc1ccccc1O. 

Breaking it down:

- 'N' represents Nitrogen.
- '\#' represents a triple bond.
- 'C' represents Carbon.
- 'c1' represents a ring (benzene ring).
- 'ccc' represents three connected carbons.
- '1' is the number of the ring.
- 'O' represents Oxygen.

So, the molecule is a Benzotriazole molecule.

In Chinese, it is written as: 
\begin{CJK*}{UTF8}{gbsn}
苯三唑
\end{CJK*}
 \\ 
        \midrule
        \addlinespace
        German & Die Molekülformel in deutscher Sprache ist:

N-(Phenyl)-acetohydrazid

Die Molekülstruktur ist ein Hydrazid, das aus einem Acetohydrazid-Molekül und einem Phenyl-Rest besteht. Der Name "N-(Phenyl)-acetohydrazid" beschreibt die Struktur des Moleküls, wobei das Acetohydrazid-Molekül an das Phenyl-Rest gebunden ist.

Eine alternative Bezeichnung für dieses Molekül ist 1-Hydroxy-2-phenyl-2-hydrazinethanon, aber "N-(Phenyl)-acetohydrazid" ist eine allgemein akzeptierte und einfache Bezeichnung.

Es ist wichtig zu beachten, dass die Molekülformel "N\#Cc1ccccc1O" eine SMILES-Notation ist, eine kurze Bezeichnung für Moleküle, die in der Chemie verwendet wird. Diese Notation kann jedoch nicht direkt als Name eines Moleküls verwendet werden.
        \\
\midrule
        \addlinespace
French & La molécule décrite par la formule chimique '' N\#Cc1ccccc1O '' est un isocyanure, plus précisément un isocyanure aromatique.

Dans la nomenclature chimique, la formule peut être décomposée comme suit :

- '' N '' représente un atome d'azote.
- Le '' \# '' indique un pont triple entre l'azote et le carbone suivant.
- '' C '' représente des atomes de carbone.
- Les '' c '' entre les atomes de carbone indiquent des liaisons entre eux.
- Le chiffre '' 1 '' entre les parenthèses indique un cycle (un anneau) composé de 6 atomes de carbone.
- '' O '' représente un atome d'oxygène.

La molécule décrite est donc un isocyanure aromatique cétogénique, qui peut être nommé '' isocyanure benzène '' ou '' isocyanure cétogénique benzénique ''.

Cependant, il est important de noter que la formule chimique donnée peut également correspondre à d
\\
\midrule
        \addlinespace
Japanese & The molecule you provided is 3-Quinuclidinone.

In Japanese, the name of this molecule is \begin{CJK*}{UTF8}{min}
3-キヌキジンオニウム
\end{CJK*} (3-Kinukijinoniu), but this is not entirely accurate, as the molecule is not an ion, but rather a ketone.

A more accurate Japanese name for this molecule would be \begin{CJK*}{UTF8}{min}
3-キヌキジノン
\end{CJK*} (3-Kinukijinon).

Here's a breakdown of the name:

- 3-: indicates the position of the carbonyl group
- \begin{CJK*}{UTF8}{min}
キヌキジ
\end{CJK*} - (Kinukiji-): refers to the quinuclidine ring
- \begin{CJK*}{UTF8}{min}
ノン
\end{CJK*} (Nōn): indicates the presence of a carbonyl group (ketone)

So, the correct Japanese name for the molecule N\#Cc1ccccc1O is \begin{CJK*}{UTF8}{min}
3-キヌキジノン
\end{CJK*}  (3-Kinukijinon).
\\
\midrule
        \addlinespace
Spanish &  La molécula descrita es un anillo aromático de benzeno (C6H6) con un grupo aminocloruro sustituido (NHCl) y un grupo hidroxilo (OH) sustituido en el anillo.

Sin embargo, considerando la notación SMILES proporcionada (N\#Cc1ccccc1O), es más probable que la molécula sea una anilina (C6H5NH2) con un grupo hidroxilo (OH) sustituido en el anillo. 

La estructura química sería: C1=CC=C(C=C1)N=O.
\\

        \bottomrule
    \end{tabular}}
    \caption{Example of molecule and descriptions in different languages generated by \texttt{Llama-3.1-8B}. }
    \label{tab:example_molecule}
\end{table*}

